GACELA -- A generative adversarial context encoder for long audio inpainting

We introduce GACELA, a generative adversarial network (GAN) designed to restore missing musical audio data with a duration ranging between hundreds of milliseconds to a few seconds, i.e., to perform long-gap audio inpainting. While previous work either addressed shorter gaps or relied on exemplars by copying available information from other signal parts, GACELA addresses the inpainting of long gaps in two aspects. First, it considers various time scales of audio information by relying on five parallel discriminators with increasing resolution of receptive fields. Second, it is conditioned not only on the available information surrounding the gap, i.e., the context, but also on the latent variable of the conditional GAN. This addresses the inherent multi-modality of audio inpainting at such long gaps and provides the option of user-defined inpainting. GACELA was tested in listening tests on music signals of varying complexity and gap durations ranging from 375~ms to 1500~ms. While our subjects were often able to detect the inpaintings, the severity of the artifacts decreased from unacceptable to mildly disturbing. GACELA represents a framework capable to integrate future improvements such as processing of more auditory-related features or more explicit musical features.

==> supplementary_friedhof.tex <==

\newpage

\section*{Supplementary Material}

\begin{figure*}[!th]
\begin{center}
	\includegraphics[width=\textwidth]{Encoder.pdf}
	\caption{Detail of the encoder network.}
	\label{fig:encoder}
\end{center}
\end{figure*}


The general structure of the network can be seen on Fig. \ref{fig:overview-network}.

\begin{figure}[!th]
\begin{center}
	\includegraphics[width=\columnwidth]{audio-inpainting-gan-v6.pdf}
	\caption{(To be moved...) Overview of the GAN structure. \nicki{Can we simplify this? It looks crazy complicated, but actually isn't}\andi{I tried}}
\label{fig:overview-network}
 \end{center}
 \end{figure}



\subsection{Parameters}
	\label{subsec:params}

The signals used for training were all sampled at 22.05 kHz. For the listening tests, the signals were resampled to 48kHz. During training, the batch size was 64. For the `normal' condition tested on every dataset, the spectrograms were split into 480 time bins, 64 time bins and 480 time bins, equating to 5.6~s, 0.74~s and 5.6~s respectively. For the `short' condition, that split was 240, 32, and 240 and for the `long' condition it was 960, 128, and 960. 
% \andi{I think this next paragraph is already covered by Section III.B}

The generator's encoder consists of 4 convolutional layers with stride 2, filters of shape 5 by 5, and number of channels 32, 64, 32, and 16, respectively. The encoded signals is flattened before being processed by a liner layer with output size 8192. After, the signal is reshaped into a rectangle and processed by 4 convolutional layer with number of channels 256, 128, 64, 32, respectively. The first two filters have shape 4 by 4 after which all filters have shape 8 by 8. Then, the signal is processed by two 32 channels residual layers with filters shaped 8 by 8. Finally, there is one last convolutional layer with 1 channel as output. The discriminator is comprised of 2 networks processing STFT signals and 3 networks processing MEL signals. Both types of network follow the same basic structure with 5 layers each, using stride 2 for each layer and filters of size 5 by 5. The main difference was in the amount of channels where the networks processing STFT signals start with 32 channels and the networks processing MEL signals start with 8 channels. After that, both networks double the amount of channels with every layer.

